Exploring the Landscape of effective field theories

In this thesis we provide new tools to determine and explore the Landscape of four-dimensional effective field theories originating from string and M-theory. The main aim is to introduce, within four-dimensional effective descriptions, elements that are predicted from string theory. To this end, a hierarchy of forms is introduced within the four-dimensional $\mathcal{N}=1$ supergravity theories. The inclusion of gauge three-forms delivers a dynamical way to generate flux-induced superpotentials. Instead, gauge two-forms, dual descriptions of axions, may be eventually gauged by three-forms to generate a superpotential coupling between the different chiral multiplet sectors of the theory. The mutual constraints among the background fluxes, such as tadpole cancellations, are imposed by gauge four-forms. A hierarchy of objects, to which the gauge forms couple, is then introduced: four-dimensional BPS-strings, membranes and 3-branes enlarge the Landscape, allowing the background fluxes to consistently change transversing different spacetime regions. The Freed-Witten anomaly cancellations and the changing of tadpole cancellation conditions due to background sources are neatly expressed by BPS-junctions of membranes ending on strings and 3-branes ending on membranes. Membrane-mediated domain wall transitions are studied, which determine how the scalar fields flow connecting a vacuum to another of the Landscape. According to the perturbative regime that is scanned only some transitions are allowed, with a dramatic influence on the spectrum of objects that can be consistently incorporated in the four-dimensional description.

==> Parts/Appendices/App_Open_String_Moduli.tex <==
\chapter{An introduction to Open String Moduli}
\label{app:Open}

==> Parts/ExtObj/ExtObj_Linear_Dual.tex <==
\section{Axions and Linear multiplets}
\label{sec:ExtObj_Axions}


Before moving on including strings in our supersymmetric theory, let us digress to recall how gauge two forms may be included into a supersymmetric action.

As stressed in Section \ref{}, two-forms appear directly among the components of linear multiplets. Remarkably, the linear multiplets do contain their three-form field strengths, making them super--field strengths for gauge two forms.

Although constrained via \eqref{}, linear multiplets contain the same amount of propagating fields as chiral multiplets, namely a real scalar (1 d.o.f) and a gauge two-form (1 d.o.f.) for the former and a complex scalar for the latter (2 d.o.f.). The na\"ive comparison of the degrees of freedom already suggests that there exists a duality which relates chiral and linear multiplets. Such a duality was introduced in \cite{} and, for the sake of completeness and to set up the notation, we will summarize here.

Preliminarily, let us consider a supersymmetric theory with some chiral superfields $\Phi^i$, $i=1, \ldots, N$, which we will here treat as spectators, and some other chiral multiplets $T^\Lambda$, $\Lambda=1,\ldots, M$. Let us assume that the K\"ahler potential does depend on $T_\Lambda$ only via their imaginary parts:
%
\be
\label{ExtObj_AL_Khyp}
K (\Phi, \bar \Phi; T) \equiv K (\Phi, \bar \Phi; \Im T)\,,
\ee
%
keeping generic the dependence on $\Phi$. The K\"ahler potential is then invariant under the \emph{axionic shifts}
%
\be
\label{ExtObj_AL_ShiftS}
T_\Lambda \rightarrow T_\Lambda + c_\Lambda
\ee
%
for real $c_\Lambda$ and we identify the lowest components $\Re T_\Lambda| = \Re t_\Lambda \equiv a_\Lambda$ as \emph{axions}, the only components influenced by the shift \eqref{ExtObj_AL_ShiftS}
%
\be
\label{ExtObj_AL_Shifta}
a_\Lambda \rightarrow a_\Lambda + c_\Lambda
\ee
%
We might therefore trade the axions $a_\Lambda$ with gauge two-forms $B_2^\Lambda$ with an electro-magnetic duality, that is
%
\be
\label{ExtObj_AL_bosdual}
\d a_\Lambda \quad \leftrightarrow \quad * \d B_2^\Lambda\,,
\ee
%
the number of degrees of freedom does not change and the shift \eqref{ExtObj_AL_Shifta} simply translates into a shift of the gauge two form $B_2 \rightarrow B_2 + \Lambda_2$ for constant two-form $\Lambda_2$.

In the same spirit as the one adopted in Chapter \ref{chapter:GSS}, we may promote the trading \eqref{ExtObj_AL_bosdual} at the superspace level passing through a first order formalism. Therefore, we first relax the assumption that in \eqref{ExtObj_AL_Khyp}, $\Im T_\Lambda$ are the imaginary parts of chiral superfields $T_\Lambda$ and rather consider them real, unconstrained superfields $U_\Lambda$.  Then, we start with the Lagrangian
%
\be
\label{ExtObj_AL_Dual1}
\call_{\rm dual} = \int \d^4 \theta K(\Phi, \bar \Phi; U) + 2 \int \d^4 \theta\, L^\Lambda U_\Lambda 
\ee
%
where $L^\Lambda$ are linear multiplets. Two paths may be followed, one leading to the ordinary formulation specified just by chiral multiplets with a K\"ahler potential \eqref{ExtObj_AL_Khyp}, the other to a dual formulation where the linear multiplets $L^\Lambda$ replace the axionic multiplets $T_\Lambda$. In details:

\begin{description}
	\item[Ordinary chiral formulation] In order to retrieve a formulation in terms of chiral multiplets only, we need to integrate out the linear multiplets $L^\Lambda$ from the Lagrangian \eqref{ExtObj_AL_Dual1}. It is clearly not possible to integrate them out directly, since they are constrained by \eqref{GSS_HF_LinConstr}. However, the constraint \eqref{GSS_HF_LinConstr} can be solved as
	%
	\be
	\label{ExtObj_AL_Dual1L}
	L^\Lambda = D^\alpha \bar D^2 \Psi_\alpha^\Lambda + \bar D_{\dot \alpha} D^2 \bar \Psi^{\Lambda\dot\alpha}
	\ee
	%
	where $\Psi^\Lambda_\alpha$, $\bar \Psi^{\Lambda \dot\alpha}$ are \emph{unconstrained} spinorial superfields. The -- now legitimate -- variations with respect to $\Psi^\Lambda_\alpha$, $\bar \Psi^{\Lambda \dot\alpha}$ of the Lagrangian \eqref{ExtObj_AL_Dual1} sets the following constraints over $U_\Lambda$:
	%
	\be
	\label{ExtObj_AL_Dual1Psi}
	\delta \Psi^\Lambda_\alpha\,, \delta \bar \Psi^{\Lambda\dot\alpha}\,: \qquad  \bar D^2 D^\alpha U_\Lambda=0\,,\quad  D^2 \bar D_{\dot\alpha} U_{\Lambda} = 0\,.
	\ee
	%
	These are solved by
	%
	\be
	\label{ExtObj_AL_Dual1U}	
	U_\Lambda = \frac{1}{2\ii} (T_\Lambda - \bar T_\Lambda ) = \Im T_\Lambda 
	\ee
	%
	for generic chiral multiplets $T_\Lambda$. Substituting \eqref{ExtObj_AL_Dual1U} into \eqref{ExtObj_AL_Dual1}, we get a Lagrangian fully depending on the chiral multiplets $\Phi$ and $T$
	%
	\be
	\label{ExtObj_AL_Dual1c}
	\call_{\rm chiral} = \int \d^4 \theta K(\Phi, \bar \Phi; \Im T)\,. 
	\ee
	%
	
	\item[Formulation with linear multiplets] The alternative formulation where the axionic multiplets $T_\Lambda$ are replaced by linear multiplets is obtained by integrating out the real multiplets $U_\Lambda$ from \eqref{ExtObj_AL_Dual1}, setting
	%
	\be
	\label{ExtObj_AL_Dual1dU}
	\delta U_\Lambda: \qquad  L^\Lambda = \frac12 \frac{\del K}{\del U_\Lambda}
	\ee
	%
	This relation does indeed provides an electro-magnetic trading as the sought one \eqref{ExtObj_AL_bosdual}. In fact, assuming for simplicity that the K\"ahler potential depends only on the axionic multiplets $T_\Lambda$, the $[D,\bar D]$--component of \eqref{ExtObj_AL_Dual1dU} relates
	%
	\be
	\d \Re t_\Lambda = - \frac12 F_{\Lambda \Sigma} *\! \d B_2^\Sigma
	\ee
	%
	Once \eqref{ExtObj_AL_Dual1dU} is plugged inside \eqref{ExtObj_AL_Dual1}, we get
	%
	\be
	\label{ExtObj_AL_Dual1Lag}
	\call_{\rm linear} = \int \d^4 \theta\, \left(K(\Phi, \bar \Phi; U) + \frac{\del K}{\del U_\Lambda}U_\Lambda \right) \equiv \int \d^4 \theta\, F(\Phi, \bar \Phi; L)
	\ee
	%
	where $F(\Phi, \bar \Phi; L)$ is the Legendre transform of the K\"ahler potential $K(\Phi, \bar \Phi; \Im T)$. The bosonic components of the Lagrangian \eqref{ExtObj_AL_Dual1Lag} are \Comment{COMPLETE}
	%
	\be
	\label{ExtObj_AL_Dual1Lagbos}
	\begin{split}
		\call_{\rm linear} |_{\rm bos} &= 
		\\
		&\quad\,+
	\end{split}
	\ee
	%
\end{description}

The procedure outlined above can be followed also in reverse: we may start with the Legendre transform \eqref{ExtObj_AL_Dual1Lag} and, by using a first order formalisms, come back to the ordinary, chiral multiplets-obly formulation. Since in the later Sections \ref{sec:Sugra_HG} and \ref{sec:Sugra_GenAct} this is the procedure that will be preferred, for the sake of completeness, we briefly show how, from \eqref{ExtObj_AL_Dual1Lag} one can obtain \eqref{ExtObj_AL_Dual1c}. We start with the first order Lagrangian
%
\be
\label{ExtObj_AL_Dual2}
\call_{\rm dual} = \int \d^4 \theta F(\Phi, \bar \Phi; L) - 2 \int \d^4 \theta\, L^\Lambda \Im T_\Lambda\,.
\ee
%
The first piece is just \eqref{ExtObj_AL_Dual1Lag} where, however, $L^\Lambda$ are real multiplets rather than linear multiplets; the second piece contains the (imaginary parts of the) chiral multiplets $T_\Lambda$ and serves for the duality. According to the formulation that we prefer, two different roads are ahead .
\begin{description}
	\item[Formulation with linear multiplets] In order to integrate out the chiral multiplets $T_\Lambda$, we first need to solve the chirality constraints $D_\alpha T_\Lambda = 0$, $\bar D^{\dot \alpha} T_\Lambda =0$ and re-express them as\footnote{\Comment{COMPLETE}}
	%
	\be
	\label{ExtObj_AL_Dual2T}
	\Im T_\Lambda = \frac{1}{2\ii} \left(\bar D^2 \bar \Xi_\Lambda - \bar D^2 \Xi_\Lambda\right)
	\ee
	%
	with $\Xi_\Lambda$ unconstrained (complex) superfields. Varying \eqref{ExtObj_AL_Dual2} with repect to $\Xi_\Lambda$, we get the constraints
	%
	\be
	\label{ExtObj_AL_Dual2U}
	\delta \Xi_\Lambda\,, \delta \bar \Xi_\Lambda\,: \qquad  D^2 L^\Lambda = 0\,,\quad \bar D^2 L^\Lambda = 0
	\ee
	%
	which tell that $U^\Lambda$ are linear multiplets, retrieving \eqref{ExtObj_AL_Dual1Lag}.
	
	\item[Ordinary chiral formulation] By integrating out the real multiplets $L^\Lambda$, we get	
	%
	\be
	\label{ExtObj_AL_Dual2L}
	\delta L^\Lambda\,: \qquad  \Im T_\Lambda = \frac12 \frac{\del F}{\del L^\Lambda}\,,
	\ee
	%
	which, plugged in \eqref{ExtObj_AL_Dual2}, allows us to re-obtain the ordinary chiral formulation:
	%
	\be
	\label{ExtObj_AL_Dual2Lag}
	\call_{\rm dual} = \int \d^4 \theta\, \left(F(\Phi, \bar \Phi; L) - \frac{\del F}{\del L^\Lambda}L^\Lambda \right) = \int \d^4 \theta\, K(\Phi, \bar \Phi; \Im T) = \call_{\rm chiral}\,.
	\ee
	%
\end{description}

==> Parts/NLPB/NLPB_Main.tex <==
\chapter{Introduction}

==> Parts/SYM/SYM_Main.tex <==
\chapter{Introduction}

==> Parts/Swampland/Swampland_Landscape_Constraints.tex <==
\section{Constraining the Landscape}




\subsection{Tadpoles in compactification EFTs}



\subsection{How many fluxes fit in an EFT?}

==> Parts/Swampland/Swampland_Landscape_Stable.tex <==
\section{Sailing through the Landscape}
\label{sec:LandSwamp_ExtObj_DW}


Some of the physical arguments that we shall introduce in the later sections rely on the possibility of changing the background fluxes by membrane--mediated transitions. As stressed for the global case in Section~\ref{sec:ExtObj_DWM}, membranes make the potential change once they are crossed, consequently modifying the space of vacua $\scrm_{\rm vac}$ in the various spacetime regions dissected by the membranes. This, in turn, leads to a change of the mass spectrum across the different spacetime regions. 

We devote this section to study how vacua can change across the spacetime. We shall focus on the case of supersymmetric domain walls, which determine \emph{stable} regions, where fields sit at certain vevs. Such a configuration is of course possible whenever a potential admits a space of vacua $\scrm_{\rm vac}$ with nontrivial zeroth homotopy group, namely it is made up by path-disconnected components. Domain walls are stable, solitonic objects which interpolate between two vacua belonging to different path-disconnected components.  

We will generalize the globally supersymmetric results of Sections~\ref{sec:ExtObj_DW} and ~\ref{sec:ExtObj_DWM} to generic supergravity theories. However, here, we directly consider the case of domain walls supported by membranes, obtaining the case without membranes as a limit thereof.


\subsection{Domain Walls in Supergravity: the flow equations and the BPS--conditions}


Let us consider a generic supergravity theory, whose matter content is described by $n$ physical chiral superfields $\Phi^i$. Our aim is to study domain walls induced by membranes, coupled to some gauge three-forms. We consider the simplest case where just a single membrane is present, covering the spacetime hypersurface $\calm= \{z=0\}$. As stressed in the previous chapters, an ordinary supergravity formulation is not fit to fully describe nontrivial couplings of the membrane to the bulk theory and we should rather consider the dual three-form formulation \eqref{Sugra_Sum_Smem}. The action\eqref{Sugra_Sum_Smem} encodes a potential via gauge three-forms; that is, in order to obtain a potential, we need to integrate out the gauge three-forms as we did in \eqref{Sugra_Sum_F4eom}. We then arrive at an `ordinary' supergravity formulation
% 
\be
\label{SL_DW_Sbos}
\begin{aligned}
	S |_{\rm bos} &=   \int_{\Sigma} \left( \frac12 \Mp^2R *1- \Mp^2 K_{i\bar \jmath} \d \varphi^i \wedge *\d \bar\varphi^{\bar \jmath}- V(\varphi,\bar\varphi) * 1 \right) 
	\\
	&\quad\,  - \int_\calm \sqrt{-\det {\bf h}}\, \calt_{\rm memb}(\varphi) + \int_{\del\Sigma} K *1
\end{aligned}
\ee
%
where the potential differs on the two sides of the membrane
%
\be
\label{SL_DW_V}
V (\varphi (z),\bar\varphi (z))= V_- (\varphi,\bar\varphi) \Theta (-z) +  V_+ (\varphi,\bar\varphi) \Theta (z) \,.
\ee
%
Working with $\caln=1$ supersymmetric theories, the potential is computed by the usual Cremmer et al. formula \eqref{Sugra_SW_Cremmeretal}, with the superpotential undertaking a step once the membrane is encountered as in \eqref{Sugra_Sum_Wpm}. The last term of \eqref{SL_DW_Sbos} is the Gibbons-Hawking-York boundary terms \cite{York:1972sj,Gibbons:1976ue,Ceresole:2006iq}, containing the extrinsic curvature $K^{\rm ext}= g^{ab} K_{ab}^{\rm ext}$ is the extrinsic curvature, with $K_{ab}^{\rm ext} =\frac12  n^m \frac{\del g_{ab}}{\del x^m}$.

Domain walls are solitonic objects, being solutions of both the Minkowskian scalar and gravitational equations of motion. In general, without further assumptions, it is pretty difficult to extract solutions of the equations of motion from the generic action \eqref{SL_DW_Sbos}. However, we are interested in the simplest family of domain wall solutions, namely \emph{flat} and \emph{static} domain walls, which enjoy an SO(1,2) symmetry along three spacetime directions. It is then useful to split the spacetime coordinates $x^m$ into $(x^i,x^3\equiv z)$, $\mu=0,1,2$. A flat domain wall fully covers the spacetime directions $x^i$ and has a nontrivial profile only along the fourth direction $z$. With respect to the globally supersymmetric case examined in the Sections~\ref{sec:ExtObj_DW} and~\ref{sec:ExtObj_DWM}, here gravity also plays a role and influences the solution. In fact, as an extended object, a domain wall `backreacts' on the spacetime metric, modifying the geometry. Compatibly with the SO(1,2) symmetry, we choose the following ansatz for the spacetime metric \cite{Vilenkin:1984hy,Cvetic:1992bf}
%
\be
\label{SL_DW_ds2}
\d s^2=e^{2D(z)}\d x^i\d x_i+\d z^2 \, ,
\ee
%
where the \emph{warping} $D(z)$ solely depends on the fourth coordinate $z$.  As a further simplifying assumption, the scalar fields $\varphi^i$ are allowed to depend only on the transverse coordinate 
\be
\label{SL_DW_varphiz}
\varphi^i=\varphi^i(z).
\ee
We assume that the scalar fields $ \varphi^i(z)$ are continuous along $z$, while their derivatives may be discontinuous at $z=0$, where the membrane is located. 


The profile of a domain wall is determined by solving some \emph{flow equations}, which dictates how the scalar fields evolve across the spacetime. We are interested in domain walls which preserve (part of) the bulk supersymmetry. The analysis that we are going to carry is pretty similar to that of domain walls in standard Supergravity (for example in \cite{Cvetic:1992bf, Cvetic:1992st, Cvetic:1992sf, Cvetic:1993xe,Cvetic:1996vr,  Ceresole:2006iq}, to which we refer for further details). In order to preserve supersymmetry, the variations of the bulk fields need to vanish over the background specified by \eqref{SL_DW_ds2}, leading to a set of Killing spinor equations. Presently, since we are focusing on bosonic domain walls, it is just sufficient to consider that the variations of the bulk fermions need to vanish.

The supersymmetry variations of the gravitino $\psi_m{}^\alpha$ and the chiralini $\chi_\alpha^i$ are
%
\be
\label{SL_DW_susy}
\begin{aligned}
	\delta \psi_m{}^\alpha &= -2 \hat{\cald}_m \epsilon^\alpha -\ii  e_m{}^c e^{-\frac{\calk}{2}} W (\varepsilon \sigma_c \bar{\epsilon})^\alpha\,,
	\\
	\delta \chi^i_\alpha &= \sqrt{2} \epsilon_\alpha e^{\frac{\calk}{2}} K^{\bar \jmath i} ( \overline{W}_{\bar \jmath}+K_{\bar \jmath}\overline{W}) -\ii \sqrt{2} \sigma_{\alpha\dot{\beta}}{}^a \bar{\epsilon}^{\dot{\beta}} \del_a \phi^i\, .
%	\\
%	\delta \rho^p_\alpha &= \sqrt{2} \epsilon_\alpha e^{\frac{\calk}{2}}\hat{K}^{\bar q p} K_{\bar q} \overline{W} -\ii \sqrt{2} \sigma_{\alpha\dot{\beta}}{}^a \bar{\epsilon}^{\dot{\beta}} \del_a t^p\,,
\end{aligned}
\ee
%
Here, $\epsilon^\alpha = \epsilon^\alpha (z)$ is the local supersymmetry parameter and the action of the covariant derivative on the supersymmetry parameter is given by 
\be
\begin{split}
	\hat{\cald}_m \epsilon^\alpha &\equiv \del_m \epsilon^\alpha + \epsilon^\beta \omega_{m\beta}{}^\alpha - \frac{\ii}{2} \cala_m \epsilon^\alpha \, ,
\end{split}
\ee
with the $U(1)$ K\"ahler connection is 
\be
\cala_m = \frac{\ii}{2} \left(K_i \del_m \phi^i - K_{\ibar} \del_m \bar{\phi}^\ibar \right)\,. 
\ee
The variations \eqref{SL_DW_susy} evaluated over the background \eqref{SL_DW_ds2} read
%
\begin{subequations}
\label{SL_DW_susydw}
\begin{align}
	\delta \psi_z{}^\alpha = & -2 \dot\epsilon^\alpha +\ii \cala_z  \epsilon^\alpha-\ii e^{\frac{\calk}{2}} W (\varepsilon \sigma_{\underline{z}} \bar{\epsilon})^\alpha\,,\label{SL_DW_susydwa}
	\\
	\delta \psi_i{}^\alpha = & e^D \left[ \dot{D}\ (\epsilon \sigma_{\underline z}\bar{\sigma}_{\iund})^\alpha - \ii e^{\frac{K}{2}} W (\varepsilon \sigma_{\iund} \bar{\epsilon})^\alpha\right]\,,\label{SL_DW_susydwb}
	\\
	\delta \chi^i_\alpha = &\sqrt{2} \epsilon_\alpha e^{\frac{\calk}{2}} K^{\bar \jmath i} ( \overline{W}_{\bar \jmath}+K_{\bar \jmath}\overline{W})  -\ii \sqrt{2} \sigma_{\alpha\dot{\beta}}{}^{\underline z} \bar{\epsilon}^{\dot{\beta}} \dot \varphi^i\, ,\label{SL_DW_susydwc}
\end{align}
\end{subequations}
%
and preserving supersymmetry requires such variations to vanish
%
\be
\label{SL_DW_susydw0}
	\delta \psi_m{}^\alpha \stackrel{!}{=} 0\,,\qquad \delta \chi^i_\alpha \stackrel{!}{=} 0\,,
\ee
%
These conditions are solved by first imposing that the local supersymmetry parameter $\epsilon_\alpha(z)$ obeys the projection conditions
\begin{important}
%
\be
\label{SL_DW_eproj}
\epsilon_\alpha (z)= \mp \ii e^{\ii\vartheta}(\sigma_{\ul 3})_{\alpha\dot\alpha}\bar\epsilon^{\dot\alpha} (z)\,,
\ee
%
\end{important}
which, plugged into \eqref{SL_DW_susydwb}-\eqref{SL_DW_susydwc}  and setting \eqref{SL_DW_susydw0}, lead to the \emph{flow equations}
\begin{important}
%
\begin{subequations}\label{SL_DW_Flow}
	\begin{align}
	\dot \varphi^i &= \mp e^{\frac 12 K(\varphi,\bar\varphi)+i\vartheta(y)}K^{\bar\jmath i}(\overline W_{\bar\jmath}+K_{\bar\jmath} \overline W)\;,\label{SL_DW_Flowa}
	\\
	\dot D &= \pm e^{\frac 12 K(\varphi,\bar\varphi)}|W| \;, \label{SL_DW_Flowb}
	\end{align}
\end{subequations}
%
\end{important}
where the dot corresponds to the derivative with respect to $z$, that is $\dot D \equiv \frac{\d }{\d z}D$, and   $\vartheta(z)= \vartheta(\varphi(z),\bar{\varphi}(z))$ is the phase of the superpotential $W$ 
namely 
\be
\label{SL_DW_vartheta} 
W=e^{\ii\vartheta}|W|\;.
\ee 
In addition to \eqref{SL_DW_Flow}, it can be shown that \eqref{SL_DW_susydwa} and \eqref{SL_DW_eproj} imply that the 
\be
\label{SL_DW_thetaflow}
\dot\vartheta=- \Im\left(\dot\varphi^i K_i\right) 
\ee
across the flow.

Some comments are in order to the crucial relations that we have found. The first of these, \eqref{SL_DW_Flowa}, in analogy with \eqref{ExtObj_DW_flow}, tells how the scalar fields evolve, passing from the vacuum $\varphi^i_{-\infty}$ at the asymptotic left of the membrane to the vacuum $\varphi^i_{+\infty}$, located at its far right. Then, \eqref{SL_DW_Flowa} is the relation determining the scalar profile of the domain wall solutions. The second relation \eqref{SL_DW_Flowb}, which do not appear in the globally supersymmetric treatment of Section~\ref{sec:ExtObj_DWM}, is connected to the geometry, expressing the backreaction of the domain wall solution, including the membrane, over the spacetime metric \eqref{SL_DW_ds2}.

We are now also in the position to describe in which sense supersymmetry is preserved. The discussion proceeds along the same lines of Section~\ref{sec:ExtObj_DWM} and here we will be very brief. The projection condition \eqref{SL_DW_eproj} tells that only half the bulk supersymmetry is preserved by the full domain wall solution. Over the membrane worldvolume, for the membrane static ground state, supersymmetry is realized via the fermionic $\kappa$--symmetry. In order to preserve half of the supersymmetry generators \emph{also} on the membrane worldvolume, we need that the supersymmetry parameter \eqref{SL_DW_eproj} is identified with the $\kappa$--symmetry parameter of \eqref{Sugra_ExtObj_Memb_kappa}. We must then require that, at $z=0$ where the membrane sits, in its ground state
\begin{important} 
	%
	\be
	\label{SL_DWM_kappa}
	\epsilon_\alpha |_{z=0} \stackrel{!}{=} \kappa_\alpha  = -\ii \frac{q_A \calv^A(\varphi)}{|q_A \calv^A(\varphi)|} \sigma^3_{\alpha \dot \alpha} \bar\kappa^{\dot \alpha} \Big|_{z=0} \;,
	\ee
	%
\end{important}
or
%
\be
\label{SL_DWM_kappab}
e^{\ii \alpha}|_{z=0} \stackrel{!}{=} \pm e^{\ii \vartheta}|_{z=0}
\ee
%
where we have defined $\vartheta \equiv \arg [q_A \calv^A(\varphi)] |_{z=0}$.

In order ti rewrite the flow equations in a more compact form, it is convenient to introduce a \emph{flowing covariantly holomorphic superpotential} \cite{Ceresole:2006iq} \footnote{Note that this quantity matches with the super-Weyl superpotential of \eqref{Sugra_SW_KWhom}, after having gauge fixed the super-Weyl compensator as in \eqref{Sugra_SW_u}.}
%
\be
\label{SL_DW_covsup}
\calz(\varphi,\bar\varphi)\equiv e^{\frac12 K(\varphi,\bar\varphi)}W=e^{\frac12 K(\varphi,\bar\varphi)}\left[\Theta(z)W_+(\varphi)+\Theta(-z)W_-(\varphi)\right]\,.
\ee
%
As in \eqref{Sugra_Sum_Wpm} and \eqref{SL_DW_V}, the dependence of $\calz$ on $z$ is both explicit, through the step functions, and implicit, through the scalar fields $\varphi^i = \varphi^i(z)$. The jump induced by the membrane over the quantity $\calz$ can be computed by taking the limits of the difference of the right and left covariantly holomorphic superpotential \eqref{SL_DW_covsup} as
%
\be
\label{SL_DW_calzjump}
\Delta\calz \equiv \lim_{\varepsilon\rightarrow  0}\left(\calz|_{z=\varepsilon}-\calz|_{z=-\varepsilon}\right)= e^{\frac12 K (\varphi,\bar\varphi)}\left(q_A \Pi^A (\varphi)\right)|_{z=0}\,.
\ee
%
The absolute value of $\Delta \calz$ is related to the (gauge-fixed) membrane tension \eqref{Sugra_ExtObj_Memb_Tmgf} as
%
\be
\label{SL_DW_effTM}
\calt_{\rm memb} \equiv 2\,e^{\frac12 K(\varphi,\bar\varphi)}\left|q_A \Pi^A(\varphi)\right|_{z=0}=2|\Delta\calz| 
\ee
%
and at $z=0$ the phase $e^{\ii\vartheta(z)}$ enters the $\kappa$-symmetry projector \eqref{Sugra_ExtObj_Memb_kappa}. 

The previous formulas may be written in a more compact way in terms of $\calz$, rather than of the superpotential $W$; the translation between the formulas makes use of the holomorphicity of $W$, which gives
%
\be
\label{SL_DW_partialmod}
\partial_{\bar{\jmath}}|W|+\ii\partial_{\bar{\jmath}}\vartheta \; |W|=0,
\ee
%
consequently relating the derivatives of $\calz$ with the K\"ahler covariant derivatives of the superpotential as
%
\be
\label{SL_DW_dZ}
\del_{\bar\jmath}|\calz|\equiv \frac12 e^{\ii\vartheta}e^{\frac12 \calk}\bar D_{\bar\jmath}\bar W\,.
\ee
%
Hence, in terms of $\calz$, the usual Cremmer et al. potential \eqref{Sugra_SW_Cremmeretal} becomes 
%
\be
\label{SL_DW_VZ}
V(\varphi,\bar\varphi) =K^{\bar\jmath i} D_i \calz \bar D_{\bar\jmath} \bar \calz - 3 |\calz|^2 = 4 K^{\bar\jmath i} \del_i |\calz| \del_{\bar \jmath} |\calz| - 3 |\calz|^2
\ee
%
and the flow equations \eqref{SL_DW_Flow} take the simpler form
\cite{Cvetic:1992bf, Cvetic:1992st, Cvetic:1992sf, Cvetic:1993xe,Cvetic:1996vr, Ceresole:2006iq}
\begin{important}
% 
\begin{subequations}
	\label{SL_DW_Flow2}
	\begin{align}
	\dot \varphi^i &= \mp 2K^{\bar\jmath i}\,\del_{\bar\jmath}|\calz|\;,\label{SL_DW_Flow2a}
	\\
	\dot D &= \pm |\calz|\;. \label{SL_DW_Flow2b}
	\end{align}
\end{subequations}
%
\end{important}



The equations \eqref{SL_DW_Flow2} govern the domain wall profile. The points where the flows start and ends are the fixed points for the \eqref{SL_DW_Flow2}. Owing to \eqref{SL_DW_dZ}, the flow equation \eqref{SL_DW_Flow2a} has fixed-point solutions provided by the supersymmetric vevs $\varphi^i_*$ (such that $D_{\bar\jmath}W|_{\varphi_*}=0$).  Then the solution of \eqref{SL_DW_Flow2b}  is $D=-|\calz_*|z+\text{constant}$, which corresponds to an AdS space of radius $1/|\calz_*|$ for $\calz_*\neq 0$ and to flat space if $\calz_*=0$. Hence, a  regular  BPS domain wall  interpolates between two different supersymmetric vacua and its geometry is asymptotically AdS or flat for $z\rightarrow\pm\infty$.      

As in AdS/CFT contexts  \cite{Girardello:1998pd,Freedman:1999gp}, one may then define a monotonic c-function which tells the direction of the flow. To this aim, let us preliminarily recall that the phase $\vartheta(z)$ is required to be a continuous function. In other words, we require the phase of $\calz$ not to change in passing through the membrane, so that we have $\Delta \calz=e^{\ii\vartheta(0)}|\Delta \calz|$. This requirement, together with the covariant holomorphicity of $\calz$ and \eqref{SL_DW_Flow2a}, implies that
\be\label{SL_DW_dcalz}
\frac{\d |\calz|}{\d z}=2\Re\left(\dot\varphi^i\del_i|\calz|\right) +\frac12 \calt_{\rm memb}\,\delta(z)\,,
\ee
which follows from \eqref{SL_DW_covsup}. As in \cite{Ceresole:2006iq}, we can combine \eqref{SL_DW_Flow2} and \eqref{SL_DW_dcalz} to get the following relation
%
\be
\label{SL_DW_Ctheorem}
\dot C=4K^{i\bar\jmath}\del_i|\calz|\del_{\bar\jmath}|\calz|+\frac12 \calt_{\rm memb}\delta(z)\geq 0 , 
\ee
%
where we have introduced $C(z)\equiv -\dot D(z)$.  Equation \eqref{SL_DW_Ctheorem} shows the contribution of the membrane to the monotonic flow of $C(z)$, which `jumps up' by $\frac12 \calt_{\rm memb}$ at $z=0$.\footnote{A similar equation was also derived in \cite{Haack:2009jg} by dimensionally reducing ten-dimensional flow equations in the presence of effective membranes corresponding to D-branes wrapped along internal cycles.}    

Let us focus on the lower sign choice in \eqref{SL_DW_Flow2}. Then,  $|\calz|_{z=+\infty}>|\calz|_{z=-\infty}$, equation \eqref{SL_DW_Flow2a} tells us that $|\calz|=C$. Hence \eqref{SL_DW_Ctheorem} also implies that $|\calz|$ monotonically increases as we move from $z=-\infty$ to $z=+\infty$. Clearly, in the case $|\calz|_{z=+\infty}<|\calz|_{z=-\infty}$, the upper choice of sign in the flow equations \eqref{SL_DW_Flow2} imply that $|\calz|$ is monotonically decreasing, while \eqref{SL_DW_Ctheorem} still holds, since in that case the sign-reversed \eqref{SL_DW_Flow2a} becomes $|\calz|=\dot D\equiv -C$. Due to this `symmetry', in the following we will just consider the \emph{lower} choice of signs in \eqref{SL_DW_eproj} and \eqref{SL_DW_Flow2}.


As a final note, let us assume to remove our assumption that $\calz$ is nowhere vanishing, supposing that $\calz|_{z_0}=0$ at some transversal coordinate $y_0$. Then, $|\calz|$ must necessarily be monotonically increasing for $z>z_0$ and decreasing for $z<z_0$, so that $\calz$ can vanish only at $z_0$. This implies that for $z>z_0$ the flow equations \eqref{SL_DW_Flow2} with the upper sign hold, while for $y<y_0$ one must use the lower signs.   






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{BPS action and domain wall tension}

We now compute the tension of the domain wall configuration enclosing the membrane. The starting point is the action \eqref{Sugra_Sum_Smem}, with membranes coupled to a bulk Supergravity action. Once gauge three-forms are set on-shell, we arrive at the action \eqref{SL_DW_Sbos}, with potential defined as in \eqref{SL_DW_Sbos}. Using the covariantly holomorphic superpotential \eqref{SL_DW_covsup}, we may rewrite \eqref{SL_DW_Sbos} as
% 
\be
\label{SL_DWT_Sbos}
\begin{aligned}
	S |_{\rm bos} &=   \int_{\Sigma} \left( \frac12 \Mp^2R *1- \Mp^2 K_{i\bar \jmath} \d \varphi^i \wedge *\d \bar\varphi^{\bar \jmath} \right) +\Mp^2 \int_{\del\Sigma} K *1
	\\
	&\quad\,- \int_\Sigma (K^{\bar\jmath i} D_i \calz \bar D_{\bar\jmath} \bar \calz - 3 |\calz|^2)*1  - \int_\calm \sqrt{-\det {\bf h}}\, \calt_{\rm memb}(\varphi,\bar\varphi) \;.
\end{aligned}
\ee
%
Now, employing the metric ansantz \eqref{SL_DW_ds2}, we get the on-shell value for the curvature
%
\be
R = - 6 \left[ (\dot D)^2 + \ddot  D \right] \,,
\ee
%
and
%
\be
\label{SL_DWT_Sbosgrav}
\begin{aligned}
	   \int_{\del\Sigma} K *1 = \frac{\d}{\d z}e^{3D} \Big|_{+\infty} - \frac{\d}{\d z} e^{3D} \Big|_{-\infty} 
\end{aligned}
\ee
%
we recognize that the `pure gravitational' part of \eqref{SL_DWT_Sbos} simply reduces to
%
\be
\frac12 \Mp^2 \int_{\Sigma} R *1+\Mp^2 \int_{\del\Sigma} K *1 = 3 \Mp^2 \int_\Sigma   (\dot D)^2\,.
\ee
%

Following \cite{Ceresole:2006iq}, we may now rewrite the action in the elegant \emph{BPS--form}
%
\be
\label{SL_DWT_SbosBPS}
\begin{aligned}
	S |_{\rm bos} &= \int\d^3 x\int\d z\, e^{3D}\left[3\big(\dot D+|\calz|\big)^2-K_{i\bar\jmath}\big(\dot\varphi^i -2K^{i\bar k}\del_{\bar k}|\calz|\big)\big(\dot{\bar\varphi}^{\bar\jmath} -2K^{l\bar \jmath}\del_l|\calz|\big)\right]
	\\
	&\quad\,-2\int\d^3 x\int\d z\, e^{3D}\left[3\dot D|\calz|+2\Re\big(\dot\varphi^i\del_i|\calz|\big)\right] 
	\\
	&\quad\,- \int \d^3x \int \d z e^{3D} \delta(z)\, \calt_{\rm memb} (\varphi,\bar\varphi)\;.
\end{aligned}
\ee
%
On the other hand, using \eqref{SL_DW_covsup} we can write the second line of \eqref{SL_DWT_SbosBPS} in the form
\be
\begin{aligned}
&-2\int\d^3 x\int\d z\,\left[ \frac{\d}{\d z}\big(e^{3D}|\calz|\big) -\frac12 \delta(z)\calt_{\rm memb} e^{3D}\right] - \int \d^3x \int \d z e^{3D} \delta(z)\, \calt_{\rm memb} 
\\
&= -2\int\d^3 x\left[\big( e^{3D}|\calz|)|_{z=+\infty}-\big(e^{3D}|\calz|\big)|_{z=-\infty}\right]\;,
\end{aligned}
\ee
where the terms localized over the membrane perfectly cancel. Then, \eqref{SL_DWT_SbosBPS} reduces to the
\be
\label{SL_DWM_redS}
\begin{aligned}
	S_{\rm red}=&\int\d^3 x\int\d z\, e^{3D}\left[3\big(\dot D+|\calz|\big)^2-K_{i\bar\jmath}\big(\dot\varphi^i -2K^{i\bar k}\del_{\bar k}|\calz|\big)\big(\dot{\bar\varphi}^{\bar\jmath} -2K^{l\bar \jmath}\del_l|\calz|\big)\right]
	\\
	&-2\int\d^3 x\left[\big( e^{3D}|\calz|)|_{z=+\infty}-\big(e^{3D}|\calz|\big)|_{z=-\infty}\right].
\end{aligned}
\ee
This reduced action is identical in form to the one obtained in \cite{Ceresole:2006iq} in the absence of membranes, basically because of the observed reciprocal cancellations of various terms localised on the membrane. 

Hence, as in the absence of membranes, the extremization of the BPS action \eqref{SL_DWM_redS} precisely reproduces the bulk flow equations \eqref{SL_DW_Flow2}. indeed, on any solution of the flow equations, we get
%
\be
\label{SL_DWM_redSos}
S_{\rm red}|_{\text{on-shell}}=-2\int\d^3 x\left[\big( e^{3D}|\calz|)|_{z=+\infty}-\big(e^{3D}|\calz|\big)|_{z=-\infty}\right]=-\int\d^3 \tilde x \,\calt_{\rm DW} , 
\ee
%
where on the slices of constant $y$ we have introduced coordinates $\tilde x^\mu=e^{D(y)}x^\mu$, so that $\d^3 \tilde x$ denotes the physical volume, and the domain wall tension is
\begin{important}
	% 
	\be
	\label{SL_DWMT}
	\calt_{\rm DW}=2\big(|\calz|_{z=+\infty}-|\calz|_{z=-\infty}\big)\;.
	\ee
	%
\end{important}



It is however important to stress that \eqref{SL_DWMT} is only formally identical to the formula obtained in the absence of membranes \cite{Cvetic:1992bf, Cvetic:1992st, Cvetic:1992sf, Cvetic:1993xe,Cvetic:1996vr, Ceresole:2006iq}. However one should keep in mind that it includes the contribution of the membrane. 
This can be seen by splitting the overall change of $|\calz|$ in the bulk and membrane contributions\footnote{In \cite{Haack:2009jg} the same conclusion was reached starting from a  ten-dimensional description of similar domain wall solutions. }
\be
\label{SL_DW_tension2}
\calt_{\rm DW}=2\big(|\calz|_{z=+\infty}-\lim_{\varepsilon\rightarrow 0}|\calz|_{z=\varepsilon}\big)+2\big(\lim_{\varepsilon\rightarrow 0}|\calz|_{z=-\varepsilon}-|\calz|_{z=-\infty}\big)+ \calt_{\rm memb}\,.
\ee


From \eqref{SL_DWMT} we see that our working assumption $|\calz|_{z=+\infty}> |\calz|_{z=-\infty}$ guarantees that $\calt_{\rm DW}>0$. The case  $|\calz|_{z=+\infty}< |\calz|_{z=-\infty}$ (with still nowhere vanishing $\calz$)  can be obtained by changing $z\rightarrow -z$ in the above steps, so that the sign-reversed flow equations \eqref{SL_DW_Flow2} extremize the corresponding BPS reduced action and the tension is given by $\calt_{\rm DW}=2\big(|\calz|_{z=-\infty}-|\calz|_{z=+\infty}\big)$. 

Furthermore, as mentioned above, at the end of the previous section, the case in which there is a vanishing point of $z_0$ of $\calz$ can be obtained by gluing two regions along which $|\calz|$ flows in opposite directions, first decreasing from $|\calz|_{z=-\infty}$ to $0$ and then increasing to $|\calz|_{z=+\infty}$. The above arguments can be easily adapted to this case as well and give  $\calt_{\rm DW}=2\big(|\calz|_{z=-\infty}+|\calz|_{z=+\infty}\big)$, again as in the absence of membranes \cite{Cvetic:1992bf, Cvetic:1992st, Cvetic:1992sf, Cvetic:1993xe,Cvetic:1996vr, Ceresole:2006iq}. However,  in this case the membrane sitting at $y_0$ would have vanishing localized tension, $\calt_{\rm DW}=0$. This would signal breaking of the validity of the effective action.   







==> Parts/Swampland/Swampland_Landscape_Unstable.tex <==
\section{Instabilities in the Landscape}


\subsection{Membrane decays, anomalies and equivalences of vacua}

x

==> Parts/Swampland/Swampland_Membranes_II.tex <==
\section{Tensionless membranes ...}





==> Parts/Swampland/Swampland_Mini-Landscape.tex <==
\section{A mini-landscape example}


To exemplify the discussion of the previous section, let us now consider a concrete simple model for which domain wall solutions can be computed explicitly. In the super-Weyl, chiral multiplet formulation the theory is described by two superfields $z^a=(z^0,z^1)$, associated with the prepotential 
\be\label{SL_DWEx_expre}
\calg=-\ii z^0 z^1.
\ee
The periods are then defined as in \eqref{Sugra_MTF_Ex_maxrank}
\be\label{SL_calvA}
\calv^A = \begin{pmatrix}
	z^0 \\ z^1 \\ -\ii z^1 \\ -\ii z^0
\end{pmatrix}\;.
\ee

The super-Weyl invariance can then be gauge-fixed by choosing, for example
\begin{equation}
\label{SL_DWEx_exfI}
	z^0 = 1\,, \qquad z^1 = - \ii \phi\,,
\end{equation}
where $\phi$ is the only physical field. The gauge-fixed potential acquires the form \eqref{Sugra_MTF_Wphys}, with $N_A = (e_0,e_1,-m^0,-m^1)$
\be\label{SL_DWEx_exSup}
W(\Phi)=(e_0+\ii m^1)-\ii (e_1 +\ii m^0)\Phi \, .
\ee

The dual three-form picture is easily identified from the discussion of Section~\ref{sec:Sugra_MTF}. We would like to dynamically generate all the constants $N_A$. We will then need, as for the maximal nonlinear case of Section~\ref{sec:Sugra_MTF_Examples}, four gauge three-forms, properly included into a couple of double three-form multiplets. Since $\calg$ is quadratic, the $2\times 2$ matrix
\be
\calg_{ab}=\ii\calm_{ab}=-\ii\left(\begin{array}{cc} 0 & 1\\
	1 & 0\end{array}\right)
\ee
is constant, and the constraint \eqref{Sugra_MTF}, which defines the two double three-form multiplets $S^a$ in terms of the complex linear superfields $\Sigma_a=(\Sigma_0,\Sigma_1)$,  becomes linear
\be
S^0= - \frac\ii2(\bar\cald^2-8\calr)\Im\Sigma_1\,,\quad S^1=-\frac\ii2(\bar\cald^2-8\calr)\Im\Sigma_0 \, . 
\ee
At the component level, they include the four three-forms
\be\label{SL_DWEx_exgauge3}
\left(\begin{array}{l} A^0_{(3)} \\
	A^1_{(3)}\\
	\tilde A_{(3)0}\\
	\tilde A_{(3)1}
\end{array}\right)
\ee
where, for clarity, we have introduced the change of notation $A^A_{3}\rightarrow A^A_{(3)}$, with field strengths $F^0_{(4)},F^1_{(4)},\tilde F_{(4)0}, \tilde F_{(4)1}$. The three-form Lagrangian is then \eqref{Sugra_MTF_L3f}, where, in the following, we will put to zero superpotential $\hat \calw$  for simplicity. 

As of now we have not assumed any particular form for the K\"ahler potential. We will regard $S^a$ as coordinates for a one-dimensional special K\"ahler manifold, whose K\"ahler potential is of the same form as \eqref{EFT_IIA_Kk}. Then, after gauge-fixing the super-Weyl invariance, we arrive at
\be\label{SL_DWEx_exKP}
K(\phi,\bar\phi)=-\log\left(4\Im\phi\right)+ \hat K_0\;.
\ee
%\be\label{SL_DWEx_excalf}
%\calf_{(4)0}=\tilde F_{(4)0}-\ii F_{(4)}^1\,,\quad \calf_{(4)1}=\tilde F_{(4)1}-\ii F_{(4)}^0 \, . 
%\ee
where $\hat K_0$ is an additional, constant contribution. In particular, we see that in order to have a well defined K\"ahler potential we should require
\be\label{SL_DWEx_phipos}
\Im\phi>0.
\ee
The three-form action has then


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bosonic action, three-forms  and $SL(2,\mathbb{Z})$ dualities}


The three-form Lagrangian may more conveniently re-written by introducing the following $SL(2,\mathbb{Z})$--covariant basis
\be\label{SL_DWEx_excalf}
\calf_{(4)0}=\tilde F_{(4)0}-\ii F_{(4)}^1\,,\quad \calf_{(4)1}=\tilde F_{(4)1}-\ii F_{(4)}^0 \, . 
\ee
and we will collect $\calf_{(4)a} =(\calf_{(4)0}, \calf_{(4)1})$. It is then possible to show that the gauge three-form action \eqref{Sugra_MTF_L3fComp_gf} reduces to
\be\label{SL_DWEx_exbaction}
S= \int_\Sigma\left[\frac12 \Mp^2 R *\!1 - \Mp^2 \frac{\d \phi \wedge *\!\d \bar\phi}{4(\Im\phi)^2} - T^{ab}(\phi) \!\bar\calf_{4a} *\!\calf_{4b}\right]+S_{\rm bd}
\ee
with the boundary contribution
\be
\label{SL_DWEx_exbactionbd}
S_{\rm bd}= \int_{\del \Sigma} (\tilde{A}_{b(3)}-\calg_{ac} A^c_{(3)}) T^{ab}  *\!\calf_{4b}+ {\rm c.c.}
\ee
and 
\be\label{SL_DWEx_excalt}
T^{ab} (\phi)= \frac{e^{-\hat K_0}}{6\,\Im\phi}\left(\begin{array}{rc} 1 {\ \ \ \ \ \ } & \ii\phi -  \Im\phi\\
	-\ii\bar\phi -  \Im\phi & |\phi|^2\end{array}\right)
\, , 
\ee
where $\hat K_0$ is the constant appearing in the complete K\"ahler potential \eqref{SL_DWEx_exKP}.
It is known that the group of symmetries associated with the special K\"ahler structure defined by the prepotential \eqref{SL_DWEx_expre} is $SL(2,\mathbb{R})$ (see for instance \cite{Freedman:2012zz}). More precisely, an element
\be
\left(\begin{array}{rr} a & b\\
	c & d\end{array}\right)\in SL(2,\mathbb{R}) 
\ee
acts on $\phi$ as follows
\be\label{SL_DWEx_phiSL2R}
\phi\rightarrow\frac{a\phi+b}{c\phi+d}\,.
\ee
In the assumption of the quantization conditions of Section~\ref{sec:Sugra_Quant}, this reduces to $SL(2,\mathbb{Z})$ (with $a,b,c,d\in\mathbb{Z}$), which we will interpret as the duality group of the model. This duality symmetry $SL(2,\mathbb{Z})$ is embedded into the group of symplectic transformations $Sp(4,\mathbb{Z})$, see e.g. \cite{Freedman:2012zz}. Here we focus on the $SL(2,\mathbb{Z})$ generators 
\be
\mathfrak{t}=\left(\begin{array}{rr} 1 & 1\\
	0 & 1\end{array}\right),\quad\mathfrak{s}=\left(\begin{array}{rr}\ 0 &\ 1\\
	-1 & 0\end{array}\right) 
\ee
which correspond to the following $Sp(4,\mathbb{Z})$ transformations
\be\label{SL_DWEx_SL2ZS}
\cals(\mathfrak{t})=\left(\begin{array}{rrrr} 1 &\ 0 &\ 0 &\ 0\\
	0 & 1 & 0 & 1\\
	-1& 0 & 1 & 0\\
	0 & 0 & 0 & 1
\end{array}\right),
\quad\cals(\mathfrak{s})=
\left(\begin{array}{rrrr} 
	0 &\ 0 &\ 1 &\ 0\\
	0 & 0 & 0 & 1\\
	-1& 0 & 0 & 0\\
	0 &-1 & 0 & 0
\end{array}\right)\,.
\ee
One can check that,  applying $\cals(\mathfrak{t})$ and $\cals(\mathfrak{s})$ to the (bosonic component of)  the symplectic vector \eqref{SL_calvA}, one gets the $\mathfrak{t}$- and $\mathfrak{s}$-actions on $\phi$ as in \eqref{SL_DWEx_phiSL2R}.\footnote{Under $\mathfrak{s}$ one needs to make also the change  $Y\rightarrow \phi Y$, which can be reabsorbed by a K\"ahler transformation $K\rightarrow K-\log\phi -\log\bar\phi$.} Furthermore, one can verify that $[\cals(\mathfrak{s})\cals(\mathfrak{t})]^3=\bbone$, which together with $\cals(\mathfrak{s})^2=-\bbone$  implies that \eqref{SL_DWEx_SL2ZS}  generate a four-dimensional representation of $SL(2,\mathbb{Z})$. 

By applying \eqref{SL_DWEx_SL2ZS} to \eqref{SL_DWEx_exgauge3}, one can then get the transformation properties of the gauge three-forms under the $SL(2,\mathbb{Z})$ duality group. Consider  the complex field-strengths \eqref{SL_DWEx_excalf} and organize them into a 2-components vector
\be\label{SL_DWEx_calfvec}
\vec\calf_{(4)}\equiv \left(\begin{array}{r}
	\calf_{(4)0}\\
	\calf_{(4)1}
\end{array}\right) \, . 
\ee
Under  $SL(2,\mathbb{Z})$ we have  $\vec\calf_{(4)}\rightarrow U\vec\calf_{(4)} $, with
\be\label{SL_DWEx_USL(2,Z)}
U(\mathfrak{t})= \left(\begin{array}{rr} 
	1 & -\ii\\
	0 & 1
\end{array}\right) 
\,,\quad 
U(\mathfrak{s})=
\left(\begin{array}{rr}
	0 & -\ii\\
	-\ii & 0\end{array}\right)\,.
\ee
Notice that these matrices satisfy $U^\dagger\sigma_1 U=\sigma_1$ and $\det U=1$, i.e.\  they are elements of $SU(1,1)$ (defined with respect to the $\mathbb{C}^2$ metric $\sigma_1$), which is known to be isomorphic to $SL(2,\mathbb{R})$. In other words,  $U(\mathfrak{t})$ and $U(\mathfrak{s})$ generate the $SU(1,1)$ representation of $SL(2,\mathbb{Z})$.

Using \eqref{SL_DWEx_excalt}, one can also check that the $2\times 2$ matrix $T^{ab}(\phi)$ transforms as follows 
\be
\begin{aligned}
	T(\phi+1)&=  U(\mathfrak{t})^{\dagger -1 } T(\phi) U(\mathfrak{t})^{-1} \, , \\
	T\Big(-\frac1\phi\Big)&=U(\mathfrak{s})^{\dagger -1 } T(\phi) U(\mathfrak{s})^{-1} \, . 
\end{aligned}
\ee
Observing that the combination $\tilde{A}_{(3)I}-\bar\calg_{IK} A^K_{(3)}$ appearing in the boundary term \eqref{SL_DWEx_exbactionbd} transforms as $\calf_{(4)I}$, one can readily check that the bulk and boundary terms in the action \eqref{SL_DWEx_exbaction} are separately invariant under the $SL(2,\mathbb{Z})$ duality group. 
This shows that the $SL(2,\mathbb{Z})$ duality group is indeed a symmetry of the action \eqref{SL_DWEx_exbaction}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The mini-landscape of vacua}
\label{SL_DWEx_sec:landscape}

Let us study the vacua of the action \eqref{SL_DWEx_exbaction} (in the absence of membranes). As discussed in Section \ref{sec:Sugra_MTF}, one can first integrate out the gauge three-forms by  picking up a particular symplectic constant vector 
\be\label{SL_DWEx_exconst}
\left(\begin{array}{c}
	m^0 \\ m^1 \\ e_0 \\ e_1\end{array}\right)\in\mathbb{Z}^4\,,
\ee
and rewriting \eqref{SL_DWEx_exbaction} in the form
\be\label{SL_DWEx_exbaction2}
S=-\int\d^4x\,e\,\left[\frac12 R+\frac{\del \phi\, \del\bar\phi}{4(\Im\phi)^2}+V(\phi,\bar\phi)\right],
\ee
where $V$ is a conventional $\caln=1$ potential 
\be\label{SL_DWEx_expot}
\begin{aligned}
	V(\phi,\bar\phi)&= e^\calk\Big(K^{\phi\bar\phi}|D_\phi W|^2-3|W|^2\Big)\\
	&=-\frac{e^{\hat K_0}}{2\Im\phi} \Big[(m^1)^2+(e_0)^2+4(m^0m^1+e_0e_1)\Im\phi 
	\\
	&\quad~~~~~~~~~~~~~~ +2(m^0e_0-m^1e_1)\Re\phi+((m^0)^2+(e_1)^2)|\phi|^2\Big]\,, 
\end{aligned}
\ee
with $\calk=K+\hat K_0$ and $W$  and $K$ are as in  \eqref{SL_DWEx_exSup} and \eqref{SL_DWEx_exKP}, respectively. Generically, the effective action \eqref{SL_DWEx_exbaction2} is not invariant under $SL(2,\mathbb{Z})$ transformations of $\phi$ (unless we  appropriately transform also the integration constants $m^a,e_a$). However, given the `microscopic' formulation with three-forms we started from, we can regard this breaking as {\em spontaneous} rather than explicit. 

Let us first consider the simplest  possibility:  $m^0=m^1=e_0=e_1=0$. In this case $W\equiv 0$ and hence $V\equiv 0$. So, we have a one-dimensional moduli space of vacua parametrized by an arbitrary expectation value of $\phi$. As standard in similar situations, one should identify two vacua related by an  $SL(2,\mathbb{Z})$  duality transformation. In view of the restriction \eqref{SL_DWEx_phipos}, the  moduli space of the inequivalent vacua can be identified with the familiar fundamental domain
\be\label{SL_DWEx_fundom}
\Big\{-\frac12\leq\Re\phi\leq \frac12\Big\}\cap \Big\{|\phi|\geq 1\Big\}\,.
\ee

On the other hand, this moduli space is drastically modified by any non-trivial set of constants \eqref{SL_DWEx_exconst}. It is useful to introduce the complex numbers
\be
\alpha_0\equiv e_0-\ii m^1\,,\quad \alpha_1\equiv e_1-\ii m^0
\ee
taking values in $\mathbb{Z}+\ii\mathbb{Z}$. Notice that the vector
\be
\vec\alpha\equiv  \left(\begin{array}{r}
	\alpha_0\\
	\alpha_1
\end{array}\right)
\ee
transforms as \eqref{SL_DWEx_calfvec} under the $SL(2,\mathbb{Z})$ duality tranformations, that is, in the fundamental $SU(1,1)$ representation generated by \eqref{SL_DWEx_USL(2,Z)}. The bosonic component of the superpotential \eqref{SL_DWEx_exSup} takes the form $W=\bar\alpha_0-\ii\bar\alpha_1\phi$ and the corresponding supersymmetric vacuum expectation value of $\phi$ (such that $D_\phi W|_{\phi_*}=0$) is 
\be\label{SL_DWEx_exvacua}
\phi_*=\ii\frac{\alpha_0}{\alpha_1}\,.
\ee
Taking into account \eqref{SL_DWEx_phipos}, we require
\be\label{SL_DWEx_exposcond}
\Im\phi_*= \frac{1}{|\alpha_1|^2}\Re(\alpha_0\bar\alpha_1) 
\ee
to be finite and positive.
In particular, this implies that the cases
$\alpha_1=0$ and $\Re(\alpha_0\bar\alpha_1)=0$ must be discarded.  
Then, given a certain $\vec\alpha$, \eqref{SL_DWEx_exvacua} is the only extremum of the potential \eqref{SL_DWEx_expot}. 

The condition $\Im\phi_*>0$ is equivalent to requiring that
\be\label{SL_DWEx_expos}
\Re(\alpha_0\bar\alpha_1)\equiv \frac12 \vec\alpha{}^\dagger \sigma_1\vec\alpha>0 . 
\ee
At the supersymmetric vacua \eqref{SL_DWEx_exvacua} the covariantly holomorphic superpotential $\calz$ takes the value
\be\label{SL_DWEx_calz*}
\calz_*=e^{\frac12\hat K_0}\frac{\bar\alpha_1}{|\alpha_1|}\sqrt{\Re(\alpha_0\bar\alpha_1)}
\ee
and the potential reduces to
\be
V_*=-3|\calz_*|^2=-3\,e^{\hat K_0}\Re(\alpha_0\bar\alpha_1)\,, 
\ee
which is strictly negative in view of \eqref{SL_DWEx_expos}, and thus determines the constant curvature of the AdS vacuum. 
The AdS radius (in natural units $M_{\rm P}=1$) is identified with the inverse of
\be\label{SL_DWEx_exmodZ}
|\calz_*|= e^{\frac12\hat K_0}\sqrt{\Re({\alpha_0\bar\alpha_1})}\, . 
\ee
Since $\alpha_0$ and $\alpha_1$ are integrally quantized, we should assume that $e^{\frac12\hat K_0}\ll 1$ in order  to be within the regime of reliability of our effective supergravity, which is equivalent to $|\calz_*|\ll 1$, therefore the AdS radius is much larger than the Planck length. 




Now the $SL(2,\mathbb{Z})$ duality group  of the theory relates a vacuum \eqref{SL_DWEx_exvacua} associated with a certain set  of constants \eqref{SL_DWEx_exconst} (and a corresponding effective superpotential \eqref{SL_DWEx_exSup}) to another vacuum associated with a different set of constants and effective superpotential. 
It follows that, chosen a certain (generic) set of constants \eqref{SL_DWEx_exconst},  the domain of  $\phi$ is the entire upper half-plane \eqref{SL_DWEx_phipos}  (up to some possible residual and non-generic identification),  and not the fundamental domain  \eqref{SL_DWEx_fundom}. This is a purely four-dimensional realization of the flux-induced monodromy effects observed in string compactifications, see for instance \cite{Marchesano:2014mla} for a recent discussion. 



\begin{figure}[h]
	\centering\includegraphics[width=7cm]{Parts/Gfx/SL2ZVacuab.pdf}
	\caption{\footnotesize A sampling of vacua \eqref{SL_DWEx_exvacua} filling the fundamental domain \eqref{SL_DWEx_fundom}, for the values of the constants $e_I,m^J \in [-11,11]$.}
	\label{fig:SL_vacua}
\end{figure}


On the other hand, in order to identify the {\em inequivalent} vacua, corresponding to inequivalent choices of the constants  \eqref{SL_DWEx_exconst} and of the corresponding effective potentials,  we can restrict ourselves to  the vacua \eqref{SL_DWEx_exvacua} which sit in the fundamental domain of \eqref{SL_DWEx_fundom}.
The set of such vacua is plotted in Fig.~\ref{fig:SL_vacua}. A similar  set of vacua appears in the simplest models of type IIB flux compactifications on a rigid Calabi--Yau  \cite{Denef:2004ze}, in which $\phi$ can be identified with the  axion-dilaton. In the type IIB models one needs to impose the tadpole cancellation condition, which adds a constraint on the set of allowed vacua. In our formulation with gauge three-forms, the tadpole cancellation condition can be implemented as outlined at the end of Section \ref{sec:Sugra_4FM}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Domain walls  between aligned vacua}
\label{SL_DWEx_sec:exDWs}

In this section we explicitly construct a class of  domain walls of the kind discussed in the previous section, relating pairs of vacua $\phi|_{-\infty}=\phi_*$ and $\phi|_{+\infty}=\phi_*'$ of the form \eqref{SL_DWEx_exvacua}, corresponding to two sets of constants $\alpha_I$ and $\alpha_I'$ respectively. We make the simplifying assumption that the phases of $\calz_*$ and $\calz'_*$ are aligned  and that the phase of  $\calz(y)$ remains constant along the flow.
Of course, in order to have a (non-trivial) domain wall  $|\calz_*|$ and $|\calz'_*|$ should be different and then the corresponding vacua cannot be related by a $SL(2,\mathbb{Z})$ duality.
From \eqref{SL_DW_thetaflow} we see that we should impose $\Im(\dot\phi\,\del_\phi K)=0$ with $K$ as in \eqref{SL_DWEx_exKP}.  This is possible only if $\Re\phi$ is constant and equals to
\be\label{SL_DWEx_exaxion}
\Re\phi_*= -\frac{\Im(\alpha_0\bar\alpha_1)}{|\alpha_1|^2} . 
\ee
Clearly, we should also require $\Re\phi_*'=\Re\phi_*$\,.
Hence, 
\be
v(y) \equiv \Im \phi(y) 
\ee
is the only dynamical real field along the flow.  Again, we will assume that $|\calz|$ is always increasing along the flow, which drives the field $v$ from $v|_{-\infty}=v_*$ towards $v|_{+\infty}=v_*'$ and, at $y=0$, it crosses a membrane of charges $p^I,q_J$ such that
\be
q_0-\ii p^1=\alpha_0-\alpha_0'\,,\quad q_1-\ii p^0=\alpha_1-\alpha'_1\,.
\ee

The equations of the flow \eqref{SL_DW_Flow2} are governed by the growth of $|\calz|$. In particular,   equation \eqref{SL_DW_Flow2a} reduces to
\be\label{SL_DWEx_flowv}
\dot{v} = 4v^2\, \frac{\d}{\d v} |\calz|\,.
\ee
For $y<0$, $|\calz|$ takes the following form
\be\label{SL_DWEx_Zv}
|\calz(v)|=\frac{e^{\frac12\hat K_0}}{2\sqrt{v}}\left[|\alpha_1|v+\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|}\right]\,.
\ee
For $y>0$ the from of $|\calz|$ is obtained by replacing $\alpha_I$ with $\alpha_I'$ in \eqref{SL_DWEx_Zv}.  


On the left of the membrane, $v_*$ is a global minimum of $|\calz|$. Hence, it is a repulsive fixed point of \eqref{SL_DWEx_flowv}, a flow is triggered and $v$ is driven away from $v_*$, letting the value of $|\calz|$ increase. When the membrane is reached at $y=0$, $v$ and consequently $|\calz|$ have evolved to certain values $v(0)$ and $|\calz|_{y=0}$. Here, the solution of the flow equations on the left should be glued to the one on the right. We are then led to impose the continuity of $v$ across $y=0$ while still keeping a growing $|\calz|$. However, since on the right of the membrane $v_*'$ is also a global minimum of $|\calz|$, $v_*'$ is a repulsive (rather than attractive) fixed point of \eqref{SL_DWEx_flowv}. Hence the solution to the flow equations is such that  $v$ reaches the value $v_*'$ at $y=0$ and then  remains constant
\be
v(y) = v_*' \quad \text{for}\;\,\,y\geq 0\,.
\ee
Correspondingly,  $|\calz|$ starts from $|\calz_*|$ at $y=-\infty$ and smoothly grows  until it reaches the membrane. At this point it jumps up to $|\calz'_*|$ and then remains constant (see Fig. \ref{fig:SL_flowZ} for an example). Hence, on the right of the membrane, the background is just the AdS vacuum solution.

Recalling 
\eqref{SL_DW_tension2}, we  see that the bound
\be\label{SL_DWEx_DZbound}
\calt_{\rm DW} \geq   \calt_{\rm memb}\,
\ee
is saturated if and only if on the left-hand side of the membrane $|\calz|$ is also constant. In the following we will first examine  the case in which the bound \eqref{SL_DWEx_DZbound} is saturated, leading to trivial flow equations on both sides of the membrane, and then we will consider an example for which the inequality \eqref{SL_DWEx_DZbound} strictly holds. 

As a warm up, 
let us assume that on the left of the membrane $\vec\alpha = 0$, so that the potential \eqref{SL_DWEx_expot} and $\calz$ are identically zero. Then, for $y<0$, the flow equations \eqref{SL_DW_Flow2} are trivial and are immediately solved by taking $v$ and $D$ to be arbitrary constants. In particular, with no loss of generality, we can choose $D(y)\equiv0$ for $y<0$. 
Therefore, on the left of the membrane, the bulk is always at a fixed Minkowski vacuum. As discussed above, on the right of the membrane, the bulk is at its supersymmetric AdS vacuum, in which $v$ takes the constant value $v_*'$. Hence, by continuity, we should impose that $v(y)\equiv v_*'$ also for $y<0$.  Furthermore, by imposing also the continuity of the warp factor, we must set $D(y)=-|\calz'_*|y$ for $y>0$. 

It is worthwhile to mention that this particular case of trivial flow for both $y < 0$ and $y > 0$ can be realized only  when on the left-hand side the vacuum is Minkowski, owing to the freedom in choosing any constant value of $v$ for $y<0$.

Let us now consider a more involved example, for which the flow on the left side of the membrane is nontrivial. For any choice of initial constants $\alpha_0,\alpha_1$ and any $k\in\mathbb{Q}$ such that
\be
k\alpha_1\in\mathbb{Z}+\ii\mathbb{Z}
\ee
we can choose a jump to new constants
\be\label{SL_DWEx_constchoice}
\alpha_0'=\alpha_0+k\alpha_1\,,\quad \alpha_1'=\alpha_1 \, , 
\ee
which clearly satisfies $\Re\phi_*'=\Re\phi_*$. Notice that
\be
\Im\phi'_*=\Im\phi_*+k\,.
\ee
The flow moves along the vertical direction of the upper-half-plane parametrized by $\phi$ (see Fig. \ref{fig:SL_FDf}). With no loss of generality, we take $k>0$, so that $\Im\phi'_*>\Im\phi_*$.   From \eqref{SL_DWEx_calz*}, one can also see that $|\calz_*'|>|\calz_*|$ which is the default  assumption in the previous section. 

\begin{figure}[h]
	\centering\includegraphics[width=6cm]{Parts/Gfx/SL2ZFD.pdf}
	\caption{\footnotesize The fundamental domain  of $\phi$. Along the domain wall, $\phi$ flows up along the vertical line specified by $\Re \phi_*$.}
	\label{fig:SL_FDf}
\end{figure}

Under these restrictions, the initial and final values of $v(y)$ are
\be
v_*=\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|^2}\,,\quad~~~~ v_*'=\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|^2}+k 
\ee
and the membranes charges are
\be\label{SL_DWEx_exMcharges}
p^0=0\,,\quad p^1=k\,\Im\alpha_1\,,\quad q_0=-k\,\Re\alpha_1\,,\quad q_1=0\,.
\ee


\begin{figure}[ht!]
	\centering\includegraphics[width=9cm]{Parts/Gfx/Simple_Example_Pot2.pdf}
	\caption{\footnotesize The potential \eqref{SL_DWEx_expot} for the choice of the constants $e_1 = m^0 =1$, $e_0 = m^1= 2$, $k=1$ and keeping $\Re\phi = 0$. The solid red line refers to the potential on the left of the membrane, while the dashed blue line to that on the right. This potential exhibits, on the left of the membrane, a supersymmetric AdS critical point located at $v_*=2$ and, on the right, a supersymmetric AdS critical point at $v_*'=3$.}
	\label{fig:SL_Example_Pot}
\end{figure}


\begin{figure}[ht!]
	\centering\includegraphics[width=8cm]{Parts/Gfx/Simple_Example_FlowZ.pdf}
	\caption{\footnotesize The flow of $|\calz|$ for the same set of parameters as in Fig. \ref{fig:SL_Example_Pot}. The solid red line refers to $|\calz|$ on the left of the membrane, while the dashed blue line to that on the right. The flow drives $v_*$ towards the value $v_*'$, at which $|\calz|$ jumps so that $v$ is located at new supersymmetric vacuum on the right.}
	\label{fig:SL_flowZ}
\end{figure}

We can now compute the function  $\calz(v,y)$ corresponding to our setting
\be
\calz(v,y)=\frac{\bar\alpha_1 e^{\frac12\hat K_0}}{2|\alpha_1|\sqrt{v}}\left[|\alpha_1| v+\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|}+k|\alpha_1|\Theta(y)\right].
\ee
In agreement with \eqref{SL_DW_dcalz}, $\calz(v,y)$ is discontinuous at $y=0$ and the width of the discontinuity is set by the tension of the membrane with the charges \eqref{SL_DWEx_exMcharges}
\be
\lim_{\varepsilon\rightarrow 0 }\Big|\calz(y_{\rm M}+\varepsilon)-\calz(y_{\rm M}-\varepsilon)\Big|=\frac{k|\alpha_1|e^{\frac12\hat K_0}}{2\sqrt{v|_{y=0}}}\equiv \frac12 T_M.
\ee
An example for the flow of $|\calz|$ is depicted in Fig. \ref{fig:SL_flowZ}. 


Consider now the flow equation \eqref{SL_DWEx_flowv}. For the examples under consideration, it takes the explicit form
\be
\dot v=e^{\frac12\hat K_0}\sqrt{v}\left[|\alpha_1|v-\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|}-k|\alpha_1|\Theta(y)\right]\label{SL_DWEx_exflow1}\, , 
\ee
which is solved by
\be
v(y)=\left\{\begin{array}{l}
	v_*\coth^2\left[\frac12|\calz_*|(y+c)\right]\quad~~\text{for $y\leq 0$} \, ,
	\\
	v_*' \quad~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\text{for $y\geq 0$} \, . 
\end{array}\right.\,
\ee
The integration constant $c$ must be negative, $c<0$, and  is fixed by the continuity at $y=0$, which imposes
%\be\label{SL_DWEx_incond}
$v_*\coth^2\left[\frac12c\,|\calz_*|\right]=v_*'
$
%\ee
and   always admits a solution.



\begin{figure}[ht]
	\centering
	\includegraphics[width=7cm]{Parts/Gfx/Simple_Example_ClassI_v} \includegraphics[width=7cm]{Parts/Gfx/Simple_Example_ClassI_Z}
	
	\centering
	\includegraphics[width=7cm]{Parts/Gfx/Simple_Example_ClassI_D} \includegraphics[width=7cm]{Parts/Gfx/Simple_Example_ClassI_R}
	
	\caption{\footnotesize Above are depicted all the solutions to the flow equations \eqref{SL_DWEx_exflow1}, \eqref{SL_DWEx_exflow2} for the same set of parameters as in Fig.\,\ref{fig:SL_Example_Pot}. The solid red lines refer to the quantities in the region on the left of the membrane, while the dashed blue lines to those on the right. On the top left there is the evolution of the scalar field: starting from the critical point on the left of the membrane, the field $v$ is driven towards the critical point on the right of the membrane. On  the  top  right  there  is  the modulus of the covariantly  holomorphic superpotential $|\calz|$, which is always increasing. On the bottom left there is the warping $D(y)$, which is always decreasing, using which the curvature, on the bottom right, can be obtained. As expected from the AdS vacua, the curvature is at a fixed positive value when the field $v$ reaches the vacua and, even though not explicitly shown here, is singular at the point $y=0$. In the figures $y$ is $|\calz_*|^{-1}$ units.}
	\label{fig:SL_Memb_Simple_Example_ClassI}
\end{figure}
Since the bulk exhibits a non-trivial flow only on the left-hand side of the membrane, the membrane tension is given by the vacuum expectation value of $\phi_*'$ to the right of the membrane 
\be
T_{\rm M}=\frac{k|\alpha_1|^2e^{\hat K_0}}{|\calz'_*|}.
\ee


We still have to solve the equation for the warping  \eqref{SL_DW_Flow2b}, which in the present case reads
\be
\dot D=-\frac{e^{\frac12\hat K_0}}{2\sqrt{v}}\left[|\alpha_1|v+\frac{\Re(\alpha_0\bar\alpha_1)}{|\alpha_1|}+k|\alpha_1|\Theta(y)\right]\label{SL_DWEx_exflow2}.
\ee
It also admits an analytic solution given by 
\be
D(y)=\left\{\begin{array}{l}
	d+{e^{-\frac12\hat K_0}\left(\log(-\sinh u)+\log\cosh u\right)}\quad~\text{for $y\leq 0$}\,,\\
	- |\calz_*'| y\quad~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\text{for $y\geq 0$}\,, 
\end{array}\right.
\ee
where we have set to zero an arbitrary additive constant  and   $u(y)\equiv\frac12 |\calz_*|(y+c)$. The integration constant $d$  is fixed by imposing the continuity of $D(y)$ at $y=0$. 


A couple of final comments. Notice that on the left-hand side of the membrane  the deviation of the complete solution from the  AdS vacuum   is concentrated within a length of the  same order of the  AdS radius $|\calz_*|^{-1}$. Hence, in this sense, the domain wall may be considered as `thick'. Furthermore, clearly, we can make a coordinate redefinition $y\rightarrow y-y_{\rm M}$ to get a solution with the membrane localised  at any point $y_{\rm M}$.  


==> Parts/Swampland/Swampland_Recap.tex <==
\section{ssss}



Perturbative regime and spectrum

==> Parts/Swampland/Swampland_Sublattice.tex <==
\section{How to choose the dynamical sublattice}


%\subsection{title}





==> Parts/Swampland/Swampland_Swampland_Program.tex <==
\section{The Swampland Program}



\subsection{Weak Gravity Conjecture}

x

\subsection{The distance conjecture}

x


\subsection{The Emergence Proposal}

x


\subsection{Intertwining the conjectures}
